VarFA: A Variational Factor Analysis Framework For Efficient Bayesian Learning Analytics

We propose VarFA, a variational inference factor analysis framework that extends existing factor analysis models for educational data mining to efficiently output uncertainty estimation in the model's estimated factors. Such uncertainty information is useful, for example, for an adaptive testing scenario, where additional tests can be administered if the model is not quite certain about a students' skill level estimation. Traditional Bayesian inference methods that produce such uncertainty information are computationally expensive and do not scale to large data sets. VarFA utilizes variational inference which makes it possible to efficiently perform Bayesian inference even on very large data sets. We use the sparse factor analysis model as a case study and demonstrate the efficacy of VarFA on both synthetic and real data sets. VarFA is also very general and can be applied to a wide array of factor analysis models.

==> full_model.tex <==
\subsection{rows and columns (full model)}
$\mY\in\mathbf{R}^{N\times Q}$ = observed data (N=number of students, Q=number of questions); $\rmC\in\mathbf{R}^{K\times N}$ = student ability factor; $\rmM\in\mathbf{R}^{K\times Q}$ question-concept association factor; $\mu\in\mathbf{R}^Q$ = question difficulty vector
\section{Related Work}
